MinConvNets: A new class of multiplication-less Neural Networks

Convolutional Neural Networks have achieved unprecedented success in image classification, recognition, or detection applications. However, their large-scale deployment in embedded devices is still limited by the huge computational requirements, i.e., millions of MAC operations per layer. In this article, MinConvNets where the multiplications in the forward propagation are approximated by minimum comparator operations are introduced. Hardware implementation of minimum operation is much simpler than multipliers. Firstly, a methodology to find approximate operations based on statistical correlation is presented. We show that it is possible to replace multipliers by minimum operations in the forward propagation under certain constraints, i.e. given similar mean and variances of the feature and the weight vectors. A modified training method which guarantees the above constraints is proposed. And it is shown that equivalent precision can be achieved during inference with MinConvNets by using transfer learning from well trained exact CNNs.

==> algo/binaried_layer.tex <==
\small{
\hspace*{\algorithmicindent} \textbf{Input}: A batch of inputs and targets $(I,Y)$, cost function $C(Y,\hat{Y})$, current weight $W^t$ and current learning rate $\eta^t$. 

\hspace*{\algorithmicindent} \textbf{Output}: updated weight $W^{t+1}$ and updated learning rate $\eta^{t+1}$.

\begin{algorithmic}[1]
  \STATE //\textbf{Forward propagation}
  \STATE $X_1 = I$
  \STATE {\textbf{for} $l=1$ \textbf{to} $L$ \textbf{do}}
  \STATE \quad \textbf{if} {$l^{th}$ layer is BB layer}
  \STATE \qquad {$\beta_{l} = \frac{1}{n}||X_{l}||_{l1}$}
  \STATE \qquad {$X_l^b = sign(X_l)$}
  \STATE \qquad {$\widetilde{X_l} = \beta_{l} X_l^b$}
  \STATE \quad \textbf{else}
  \STATE \qquad {$\widetilde{X_l} = X_l$}
  
  \STATE \quad \textbf{if} {$l^{th}$ layer is HB layer or BB layer}
  \STATE \qquad\textbf{for} $k^{th}$ filter in $l^{th}$ layer \textbf{do}
  \STATE \qquad\quad$\alpha_{lk} = \frac{1}{n}||W^t_{lk}||_{l1}$
  \STATE \qquad\quad$W^B_{lk} = sign(W^t_{lk})$
  \STATE \qquad\quad$\widetilde{W}_{lk} = \alpha_{lk}W^B_{lk}$
  \STATE \quad \textbf{else}
  \STATE \qquad$\widetilde{W}_{lk} = W_{lk}$
  \STATE \quad$X_{l+1}=$\textbf{Forward}$(\widetilde{X_l},\widetilde{W}_l,l)$
  \STATE $\hat{Y} = X_{L+1}$

  \STATE //\textbf{Backward propagation}
  \STATE $\frac{\partial{C}}{\partial{\widetilde{W}}}=$\textbf{Backward}$(\frac{\partial{C}}{\partial{\hat{Y}}},\widetilde{W})$
  \STATE $W^{t+1}=$\textbf{UpdateParamters}$(W^t,\frac{\partial{C}}{\partial{\widetilde{W}}},\eta^t)$
  \STATE $\eta^{t+1}=$\textbf{UpdateLearningrate}$(\eta^t,t)$
  \end{algorithmic}
  
}

==> algo/pythoncode/L_intergral.tex <==
import numpy as np
import matplotlib.pyplot as plt

n=400

def one_d_gaussian(x,mu,sigma):
    N = np.sqrt(2*np.pi*np.power(sigma,2))
    fac = np.power(x-mu,2)/np.power(sigma,2)
    return np.exp(-fac/2)/N

def p_x(x,x_mean,x_var):
    return one_d_gaussian(x,x_mean,x_var)

def p_w(w,w_mean,w_var):
    return one_d_gaussian(w,w_mean,w_var)

def fh(x,w):
    return np.abs(x*w)

def fg(x,w):
    return np.minimum(np.abs(x),np.abs(w))


def update_array(k,v):
    x_mean = k
    x_var = v
    
    w_mean = k
    w_var = v
    x_line = np.linspace(x_mean-4*x_var, x_mean+4*x_var, n+1)
    w_line = np.linspace(w_mean-4*w_var, w_mean+4*w_var, n+1)
    s = (x_line[1]-x_line[0])*(w_line[1]-w_line[0])
    r = (x_line[1]-x_line[0])

    area = (n,n)
    hv = np.zeros(area)
    gv = np.zeros(area)
    p_hgv = np.zeros(area)
    for i in range(n):
        for j in range(n):
            x = x_line[i]
            w = w_line[j]
            hv[i,j] = fh(x,w)
            gv[i,j] = fg(x,w)
            p_hgv[i,j]= p_x(x, x_mean, x_var)*p_w(w, w_mean, x_var)

    h_mean = 0
    g_mean = 0
    for i in range(n):
        for j in range(n):
            h_mean += hv[i,j]*s*p_hgv[i,j]
            g_mean += gv[i,j]*s*p_hgv[i,j]
    return x_line, w_line, s, r, hv, gv, p_hgv, h_mean, g_mean

def func(p,q,pm,qm):
    return np.abs(1.0*(q-p)/(p))

def loss(p, q, s, r, pm, qm, p_hgv):
    eps = 0.25*s
    L = 0
    for i in range(n-1):
        for j in range(n-1):
            #if p[i,j] == 0 or p[i+1,j]==0 or p[i,j+1]==0 or p[i+1,j+1]==0:
            #    continue
            f = 0
            cnt = 4
            if p[i,j] > eps:
                f += func(p[i,j],q[i,j],pm,qm)           #np.fabs(1.0*(p[i,j]-q[i,j])/q[i,j])
            else:
                cnt = cnt-1
            if p[i+1,j] > eps:
                f += func(p[i+1,j],q[i+1,j],pm,qm)           #np.fabs(1.0*(p[i,j]-q[i,j])/q[i,j])
            else:
                cnt = cnt-1
            if p[i,j+1] > eps:
                f += func(p[i,j+1],q[i,j+1],pm,qm)           #np.fabs(1.0*(p[i,j]-q[i,j])/q[i,j])
            else:
                cnt = cnt-1
            if p[i+1,j+1] > eps:
                f += func(p[i+1,j+1],q[i+1,j+1],pm,qm)           #np.fabs(1.0*(p[i,j]-q[i,j])/q[i,j])
            else:
                cnt = cnt-1
            #f2 =func(p[i+1,j],q[i+1,j],pm,qm)       #np.fabs(1.0*(p[i+1,j]-q[i+1,j])/q[i+1,j])
            #f3 =func(p[i,j+1],q[i,j+1],pm,qm)       #np.fabs(1.0*(p[i,j+1]-q[i,j+1])/q[i,j+1])
            #f4 =func(p[i+1,j+1],q[i+1,j+1],pm,qm)   #np.fabs(1.0*(p[i+1,j+1]-q[i+1,j+1])/q[i+1,j+1])
            if cnt != 0:
                f = 1.0*f/cnt
            else:
                #print("p:"+str(p[i,j])+"p:"+str(p[i,j+1])+"p:"+str(p[i+1,j+1])+"e:"+str(eps))
                continue
            v = f*s
            L += v*p_hgv[i,j]
    return L

def cov(p, q, s, p_mean, q_mean, p_hgv):
    c = 0
    for i in range(n-1):
        for j in range(n-1):
            f1 = (p[i,j]-p_mean)      *(q[i,j]-q_mean)
            f2 = (p[i,j+1]-p_mean)    *(q[i,j+1]-q_mean)
            f3 = (p[i+1,j]-p_mean)    *(q[i+1,j]-q_mean)
            f4 = (p[i+1,j+1]-p_mean)  *(q[i+1,j+1]-q_mean)
            f = 0.25*(f1+f2+f3+f4)
            v = f*s
            c += v*p_hgv[i,j]
    return c

k_line = np.zeros(40)
l_line = np.zeros(40)
for cnt in range(40):
    k=0.05*cnt
    v=1.8
    x_line, w_line, s, r, hv, gv, p_hgv, h_mean, g_mean = update_array(k,v)
    l=loss(hv,gv,s,r,h_mean,g_mean,p_hgv)
    k_line[cnt] = k
    l_line[cnt] = l
    print(k,l)

plt.plot(k_line,l_line)
plt.show()

#for vcnt in range(100):
#    v=0.02*(vcnt+1)
#    l_min = 100
#    k_min = 0
#    c_min = 0
#    for kcnt in range(200):
#        k=0.01*(kcnt)
#        x_line, w_line, s, r, hv, gv, p_hgv, h_mean, g_mean = update_array(k,v)
#        l = loss(hv,gv,s,r,h_mean,g_mean,p_hgv)
#        c1 = cov(hv,gv,s,h_mean,g_mean,p_hgv)
#        v1 = cov(hv,hv,s,h_mean,h_mean,p_hgv)
#        v2 = cov(gv,gv,s,g_mean,g_mean,p_hgv)
#        c = 1.0*c1/np.sqrt(v1*v2)
#        if l<l_min:
#            l_min = l
#            k_min = k
#            c_min = c
#    print(v,k_min,c_min,l_min)

==> figure/ac_mult.tex <==
\begin{circuitikz}
\huge 
\draw (0, 5.5)node[and port] (and1){}
(0, 4)node[and port] (and2){}
(0, 2)node[and port] (and3){}
(0, 0.5)node[and port] (and4){}
(2, 3)node[or port] (or){}


(and1.in 1) node[left=1.5cm](a1) {a[1]}
(and1.in 2) node[left=1.5cm](b1) {b[1]}

(and4.in 1) node[left=1.5cm](a0) {a[0]}
(and4.in 2) node[left=1.5cm](b0) {b[0]}

(and1.out) node[right=2cm](c2) {c[2]}
(or.out) node[right=0cm](c1) {c[1]}
(and4.out) node[right=2cm](c0) {c[0]}

%(a1.east) to[short,-*] (and1.in 1) |- (and3.in 1)

(a1.east) to[short,-*] ( $(a1.east)!.7!(and1.in 1)$ ) coordinate (branch)
    -- (and1.in 1)
(branch) |- (and3.in 1)

(b1.east) to[short,-*] ( $(b1.east)!.3!(and1.in 2)$ ) coordinate (branch)
    -- (and1.in 2)
(branch) |- (and2.in 1)

(a0.east) to[short,-*] ( $(a0.east)!.3!(and4.in 1)$ ) coordinate (branch)
    -- (and4.in 1)
(branch) |- (and2.in 2)

(b0.east) to[short,-*] ( $(b0.east)!.7!(and4.in 2)$ ) coordinate (branch)
    -- (and4.in 2)
(branch) |- (and3.in 2)

(and2.out) |- (or.in 1)
(and3.out) |- (or.in 2)

(and1.out) -- (c2)
(or.out) -- (c1)
(and4.out) -- (c0)

%(0, 7)node[xnor port] (xnor){}
%
%(xnor.in 1) node[left=1.5cm](as) {a[s]}
%(xnor.in 2) node[left=1.5cm](bs) {b[s]}
%(xnor.out) node[right=2cm](cs) {c[s]}
%
%(as) -- (xnor.in 1)
%(bs) -- (xnor.in 2)
%(xnor.out) -- (cs)



;
%(b0.east) to[short,-*] (and4.in 2) |- (and3.in 2);
\end{circuitikz}

%\begin{tikzpicture}[circuit logic US]
%     %\node[and gate, inputs={normal,inverted,normal,inverted}] (A) {};
%\node (a1) at (0,9) {a1}; 
%\node (b1) at (0,7) {b1}; 
%\node (a0) at (0,3) {a0}; 
%\node (b0) at (0,1) {b0}; 
%
%\node[and gate] (and1) at (2,8) {and};
%\node[and gate] (and2) at (2,6) {and};
%\node[and gate] (and3) at (2,4) {and};
%\node[and gate] (and4) at (2,2) {and};
%
%\node[or gate] (or1) at (5,5) {or};
%
%\node (c2) at (7,8) {c2}; 
%\node (c1) at (7,5) {c1}; 
%\node (c0) at (7,2) {c0}; 
%
%\draw (a1.east) -- ++(right:3mm) |- (and1.input 1);
%\draw (b1.east) -- ++(right:3mm) |- (and1.input 2);
%
%\draw (b1.east)  -- ++(right:5mm) |- (and2.input 1);
%\draw (a0.east)  -- ++(right:5mm) |- (and2.input 2);
%
%\draw (a1.east)  -- ++(right:7mm) |- (and3.input 1);
%\draw (b0.east)  -- ++(right:7mm) |- (and3.input 2);
%
%\draw (a0.east)  -- ++(right:3mm) |- (and4.input 1);
%\draw (b0.east)  -- ++(right:3mm) |- (and4.input 2);
%
%
%
%%\matrix[column sep=14mm]
%%{
%%\node (a0) {a0}; & \node [and gate] (a1) {and}; & & \node (c0) {c0};\\
%%\node (b0) {b0}; &  & \\
%%& \node [and gate] (a2) {and}; & \\
%%& &  \node [or gate] (o1) {or};\\
%%& \node [and gate] (a3) {and}; & \\
%%\node (a1) {a1}; & \node [and gate] (a4) {and}; & \\
%%\node (b1) {b1}; &  & \\
%%};
%%\draw (i0.east) -- ++(right:3mm) |- (a1.input 1);
%%\draw (i1.east) -- ++(right:3mm) |- (a1.input 2);
%%\draw (i1.east) -- ++(right:3mm) |- (a2.input 1);
%%\draw (i2.east) -- ++(right:3mm) |- (a2.input 2);
%%\draw (a1.output) -- ++(right:3mm) |- (o.input 1);
%%\draw (a2.output) -- ++(right:3mm) |- (o.input 2);
%%\draw (o.output) -- ++(right:3mm);
%
%\end{tikzpicture}

==> others/multi_matrix.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp12474397937043169] 
\draw   (77,112) -- (147,112) -- (147,250) -- (77,250) -- cycle ;
%Shape: Rectangle [id:dp874661144883466] 
\draw   (515.33,110.18) -- (516.01,249.33) -- (378.5,250) -- (377.82,110.85) -- cycle ;
%Shape: Rectangle [id:dp5130009905773703] 
\draw   (336.61,148.24) -- (337.38,218.24) -- (199.39,219.76) -- (198.62,149.76) -- cycle ;

% Text Node
\draw (112,101) node  [align=left] {$\displaystyle f_{h}$x$\displaystyle f_{w}$xC};
% Text Node
\draw (66,182) node [rotate=-270] [align=left] {HxW};
% Text Node
\draw (187,181) node [rotate=-270] [align=left] {$\displaystyle f_{h}$x$\displaystyle f_{w}$xC};
% Text Node
\draw (259,138) node  [align=left] {$ $C$\displaystyle _{out}$};
% Text Node
\draw (447,100) node  [align=left] {$ $C$\displaystyle _{out}$};
% Text Node
\draw (371,166) node [rotate=-270] [align=left] {HxW};
% Text Node
\draw (158,180) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {\textbf{{\large X}}};
% Text Node
\draw (348,174) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {{\large \textbf{=}}};
% Text Node
\draw (109,268) node [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {Matrix$\displaystyle _{input}$};
% Text Node
\draw (255,267) node [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {Matrix$\displaystyle _{weights}$};
% Text Node
\draw (438,269) node [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {Matrix$\displaystyle _{result}$};


\end{tikzpicture}


==> others/ouessant.tex <==
\begin{tabular}{|c|c|}
\hline
\# processor & 2 \\ \hline
Model &	POWER8+	\\ \hline
Core & 10 \\ \hline
Logical cores & 10-80 \\ \hline
Frequency &	2.86 GHz \\ \hline
Memory & 128 GB \\ \hline
Memory controller &	2 \\ \hline
L3 Cache&	8 MB \\ \hline
L4 Cache&	16 MB \\ \hline
Memory bandwidth&	230 GB/s \\ \hline
Performance peak&	235 GFlop/s \\ \hline
\# GPUs&	4 \\ \hline
Model&	Tesla P100 \\ \hline
CUDA cores&	3584 \\ \hline
Memory&	16 GB \\ \hline
Performance peak&	5.3 Tflop/s \\ \hline
% \input{ouessant.tex}
\end{tabular}


==> others/table1.tex <==
224	&	224	&	9	&	3	&	16	&		16	&	1 \\ \hline
112	&	112	&	9	&	16	&	32	&		16	&	2 \\ \hline
56	&	56	&	9	&	32	&	64	&		16	&	4 \\ \hline
28	&	28	&	9	&	64	&	128	&		16	&	8 \\ \hline
14	&	14	&	9	&	128	&	256	&		16	&	16 \\ \hline
7	&	7	&	9	&	256	&	512	&		16	&	32 \\ \hline
7	&	7	&	9	&	512	&	1024	&	16	&	64 \\ \hline
7	&	7	&	9	&	1024&	1024	&	16	&	64 \\ \hline
7	&	7	&	1	&	1024&	90	&	16	&	6 \\ \hline


==> others/tiny_yolo.tex <==
		\begin{tabular}{c|c|c}
	        	\textbf{Tiny-YOLO} & Filters & Size / Stride \\
		        \hline
	            Convolutional & 16 & 3 x 3 / 1 \\
	            Maxpool & 	& 2 x 2 / 2 \\
	            Convolutional & 32 & 3 x 3 / 1 \\
	            Maxpool & 	& 2 x 2 / 2 \\
	            Convolutional & 64 & 3 x 3 / 1 \\
	            Maxpool & 	& 2 x 2 / 2 \\
	            Convolutional & 128 & 3 x 3 / 1 \\
	            Maxpool & 	& 2 x 2 / 2 \\
	            Convolutional & 256 & 3 x 3 / 1 \\
	            Maxpool & 	& 2 x 2 / 2 \\
	            Convolutional & 512 & 3 x 3 / 1 \\
	            Maxpool & 	& 2 x 2 / 1 \\
	            Convolutional & 1024 & 3 x 3 / 1 \\
                Convolutional & 1024 & 3 x 3 / 1 \\
        	    Convolutional & 90 & 1 x 1 / 1 \\
    	        Detection &&  
	        \end{tabular}


==> table/ac_mult.tex <==
\begin{tabular}{c||c|c|c|c}
$\times$& 0 & 1 & 2 & 3  \\\hline\hline
0 & 0 & 0 & 0 & 0 \\\hline
1 & 0 & 1 & 2 & 3 \\\hline
2 & 0 & 2 & 4 & 6 \\\hline
3 & 0 & 3 & 6 & \textcolor{red}{7}
\end{tabular}


==> table/generalize.tex <==
%    \begin{tabular}{c|c|c|c}
%         IOU(\%)/ mAP & YOLOv2 & Quad & Quad-Approx \\ \hline
%         SDC-2018~\cite{xu2019dac} & 70.17/90.20 & 62.43/ 80.52 & 62.14/80.33\\ \hline
%         COCO-2017~\cite{lin2014microsoft} & 43.28/37.77 & 40.52/ 30.90 & 40.50/30.82\\ \hline
%         Pascal VOC~\cite{everingham2010pascal}& 66.25/80.07 & 60.98/76.94 & 60.95/76.08  
%    \end{tabular}

    \begin{tabular}{c|c|c|c}
         mAP (\%) & YOLOv2 & Quad & Quad-Approx \\ \hline
         SDC-2018~\cite{xu2019dac} & 90.20 & 80.52 & 80.33\\ \hline
         COCO-2017~\cite{lin2014microsoft} & 37.77 & 30.90 & 30.82\\ \hline
         Pascal VOC~\cite{everingham2010pascal}& 80.07 & 76.94 & 76.08  
    \end{tabular}

%
%    \begin{tabular}{c|c|c|c|c|c|c}
%         Network & \multicolumn{2}{c}{YOLOv2} & \multicolumn{2}{|c}{Quad}  & \multicolumn{2}{|c}{Quad-Approx} \\ \hline
%         Evaluation Criteria & IOU & mAP & IOU & mAP & IOU & mAP\\ \hline
%         SDC-2018~\cite{xu2019dac} & 70.17 & 90.20 & 62.43 & 80.52 & 62.14 &80.33\\ \hline
%         COCO-2017~\cite{lin2014microsoft} & 43.28 & 37.77 & 40.52 & 30.90 & 40.50&30.82\\ \hline
%         Pascal VOC~\cite{everingham2010pascal}& 66.25 & 80.07 & 60.98 & 76.94 & 60.95 & 76.08  
%    \end{tabular}


==> table/hardware.tex <==
%   \begin{tabular}{c|c|c|c}
%         Type & Normal & Quad & Quad-Approx \\ \hline
%         LUT & 21089 /708x3  & 20705 / 430x3  & 24311 / 1612x3 \\ \hline
%         LUT & 21089 /708x3  & 20705 / 430x3  & 24311 / 1612x3 \\ \hline
%         LUT & 21089 /708x3  & 20705 / 430x3  & 24311 / 1612x3 \\ \hline
%         FF & 17587  / 1275x3 & 14362 / 775x3 &  16606 / 1333x3\\ \hline
%         DSP & 123  / 16x3 & 127 /16x3 & 79 / 0x3  \\ \hline
%         Bram(18K) & 122  & 85  &  97 \\ \hline
%         Cycle & 5 & 5 & 7 \\ \hline
%         execution(4ns / 2ns) & 345997500 ps / 146747 ns & 345997500 ps / 146747 ns & 345997500 ps   / 146775 ns
%    \end{tabular}


==> table/mixed_arch.tex <==
\small{		\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
	        	Conv Layer & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
		        \hline
	            HH-ALL & HH & HH & HH & HH & HH & HH & HH & HH & HH\\ 
		        \hline
	            HB-ALL & HB & HB & HB & HB & HB & HB & HB & HB & HB\\ 
                \hline
	            BB-1    & \textcolor{cyan}{BB} & HB & HB & HB & HB & HB & HB & HB & HB \\
	            BB-2    & HB & \textcolor{cyan}{BB} & HB & HB & HB & HB & HB & HB & HB \\
	            BB-3    & HB & HB & \textcolor{cyan}{BB} & HB & HB & HB & HB & HB & HB \\
	            BB-4    & HB & HB & HB & \textcolor{cyan}{BB} & HB & HB & HB & HB & HB \\
	            BB-5    & HB & HB & HB & HB & \textcolor{cyan}{BB} & HB & HB & HB & HB \\
	            BB-6    & HB & HB & HB & HB & HB & \textcolor{cyan}{BB} & HB & HB & HB \\
	            BB-7    & HB & HB & HB & HB & HB & HB & \textcolor{cyan}{BB} & HB & HB \\
	            BB-8    & HB & HB & HB & HB & HB & HB & HB & \textcolor{cyan}{BB} & HB \\ 
                \hline
	            BB-1,2    & \textcolor{cyan}{BB} & \textcolor{cyan}{BB} & HB & HB & HB & HB & HB & HB & HB \\
	            BB-3,4   & HB & HB & \textcolor{cyan}{BB} & \textcolor{cyan}{BB} & HB & HB & HB & HB & HB \\
	            BB-5,6   & HB & HB & HB & HB & \textcolor{cyan}{BB} & \textcolor{cyan}{BB} & HB & HB & HB \\
	            BB-7,8   & HB & HB & HB & HB & HB & HB & \textcolor{cyan}{BB} & \textcolor{cyan}{BB} & HB \\
	        \end{tabular}
}


==> table/resource.tex <==
%    \begin{tabular}{c|c|c|c}
%         Type & Normal & Quad & Quad-Approx \\ \hline
%         LUT & 21089 /708x3  & 20705 / 430x3  & 24311 / 1612x3 \\ \hline
%         FF & 17587  / 1275x3 & 14362 / 775x3 &  16606 / 1333x3\\ \hline
%         DSP & 123  / 16x3 & 127 /16x3 & 79 / 0x3  \\ \hline
%         Bram(18K) & 122  & 85  &  97 \\ \hline
%         Cycle & 5 & 5 & 7 \\ \hline
%         execution(4ns / 2ns) & 345997500 ps / 146747 ns & 345997500 ps / 146747 ns & 345997500 ps   / 146775 ns
%    \end{tabular}


==> table/tiny_yolo.tex <==
%		\begin{tabular}{c|c|c}
%	        	\textbf{Tiny-YOLO} & Filters & Size / Stride \\
%		        \hline
%	            Convolutional & 16 & 3 x 3 / 1 \\
%	            Maxpool & 	& 2 x 2 / 2 \\
%	            Convolutional & 32 & 3 x 3 / 1 \\
%	            Maxpool & 	& 2 x 2 / 2 \\
%	            Convolutional & 64 & 3 x 3 / 1 \\
%	            Maxpool & 	& 2 x 2 / 2 \\
%	            Convolutional & 128 & 3 x 3 / 1 \\
%	            Maxpool & 	& 2 x 2 / 2 \\
%	            Convolutional & 256 & 3 x 3 / 1 \\
%	            Maxpool & 	& 2 x 2 / 2 \\
%	            Convolutional & 512 & 3 x 3 / 1 \\
%	            Maxpool & 	& 2 x 2 / 1 \\
%	            Convolutional & 1024 & 3 x 3 / 1 \\
%                Convolutional & 1024 & 3 x 3 / 1 \\
%        	    Convolutional & 90 & 1 x 1 / 1 \\
%    	        Detection &&  
%	        \end{tabular}
%
%        \begin{tabular}{c|c|c|r}
%        	Type & Filters & Size / Stride &Output\\
%        \hline
%            Input &&&416 x 416 x 3\\
%            Convolutional & 16 & 3 x 3 / 1 & 416 x 416 x 16 \\
%            Maxpool & 	& 2 x 2 / 2 & 208 x 208 x 16 \\
%            Convolutional & 32 & 3 x 3 / 1 & 208 x 208 x 32 \\
%            Maxpool & 	& 2 x 2 / 2 & 104 x 104 x 32 \\
%            Convolutional & 64 & 3 x 3 / 1 & 104 x 104 x 64 \\
%            Maxpool & 	& 2 x 2 / 2 & 52 x 52 x 64 \\
%            Convolutional & 128 & 3 x 3 / 1 & 52 x 52 x 128 \\
%            Maxpool & 	& 2 x 2 / 2 & 26 x 26 x 128 \\
%            Convolutional & 256 & 3 x 3 / 1 & 26 x 26 x 256 \\
%            Maxpool & 	& 2 x 2 / 2 & 13 x 13 x 256 \\
%            Convolutional & 512 & 3 x 3 / 1 & 13 x 13 x 512 \\
%            Maxpool & 	& 2 x 2 / 1 & 13 x 13 x 512 \\
%            Convolutional & 1024 & 3 x 3 / 1 & 13 x 13 x 1024 \\
%            Convolutional & 1024 & 3 x 3 / 1 & 13 x 13 x 1024 \\
%            Convolutional & 90 & 1 x 1 / 1 & 13 x 13 x 90 \\
%            Detection &&&
%        \end{tabular}
        		\begin{tabular}{|c|c|c|c|c|c|} 
\hline
\multicolumn{5}{|c|}{General} & PACT\\ \hline
	        Type &	H x W & C & $ f_h$ x $f_w $ / $S$ & $N$  & $\alpha_x$\\ \hline
Conv.   & 416 x 416  &   3   &  3 x 3 / 1    &	16   &	    \\ \hline
Maxpool & 416 x 416  &   16  &  2 x 2 / 2    &  16   &	    \\ \hline
Conv.   & 208 x 208  &   16  &  3 x 3 / 1    &	32   &	54	\\ \hline
Maxpool & 208 x 208  &   32  &  2 x 2 / 2    &  32   &		\\ \hline
Conv.   & 104 x 104  &   32  &  3 x 3 / 1    &	64   &	27	\\ \hline
Maxpool & 104 x 104  &   64  &  2 x 2 / 2    &  64   &	    \\ \hline
Conv.   &  52 x  52  &   64  &  3 x 3 / 1    &	128  &	18	\\ \hline
Maxpool &  52 x  52  &   128 &  2 x 2 / 2    &  128  &		\\ \hline
Conv.   &  26 x  26  &   128 &  3 x 3 / 1    &	256  &	12	\\ \hline
Maxpool &  26 x  26  &   256 &  2 x 2 / 2    &  256  &		\\ \hline
Conv.   &  13 x  13  &   256 &  3 x 3 / 1    &	512  &	7.5	\\ \hline
Maxpool &  13 x  13  &   512 &  2 x 2 / 1    &  512  &		\\ \hline
Conv.   &  13 x  13  &   512 &  3 x 3 / 1    &	1024 &	6	\\ \hline
Conv.   &  13 x  13  &   1024&  3 x 3 / 1    &	1024 &	6	\\ \hline
Conv.   &  13 x  13  &   1024&  1 x 1 / 1    &	90   & 		\\ \hline
	        \end{tabular}                               


==> table/tiny_yolo_params.tex <==
%		\begin{tabular}{c|c|c|c|c|c|c|c}
%	        \# Conv. &	H & W & $ f_h \times f_w $ & C & $C_{out}$ & $N_{lanes}$ & $N_{iter}$ \\ \hline
%1&	224	&	224	&	9	&	3	&	16		&		16	&	1  \\ 
%2&	112	&	112	&	9	&	16	&	32		&		16	&	2  \\
%3&	56	&	56	&	9	&	32	&	64		&		16	&	4  \\ 
%4&	28	&	28	&	9	&	64	&	128		&		16	&	8  \\ 
%5&	14	&	14	&	9	&	128	&	256		&		16	&	16 \\
%6&	7	&	7	&	9	&	256	&	512		&		16	&	32 \\ 
%7&	7	&	7	&	9	&	512	&	1024	&		16	&	64 \\ 
%8&	7	&	7	&	9	&	1024&	1024	&		16	&	64 \\ 
%9&	7	&	7	&	1	&	1024&	90		&		16	&	6  \\ 
%	        \end{tabular}
	
		\begin{tabular}{c|c|c|c|c|c|c|c}
	        \# Conv. &	H & W & $ f_h \times f_w $ & C & $C_{out}$ & $N_{lanes}$ & $N_{iter}$ \\ \hline
1&  416	&   416	&  3x3   &3	    &	16  &   32	&	1  \\ 
2&  208	&   208	&  3x3   &16    &	32  &   32	&	1  \\
3&  104	&   104	&  3x3   &32    &	64  &   32	&	2  \\ 
4&  52  &   52  &  3x3   &64    &	128 &   32	&	4  \\ 
5&  26  &   26  &  3x3   &128   &	256 &   32	&	8 \\
6&  13  &   13  &  3x3   &256   &	512 &   32	&	16 \\ 
7&  13  &   13  &  3x3   &512   &	1024&   32	&	32 \\ 
8&  13  &   13  &  3x3   &1024  &	1024&   32	&	32 \\ 
9&  13  &   13  &  1x1   &1024  &	90  &   32	&	3  \\ 
	        \end{tabular}


==> table/utilization.tex <==
%\begin{tabular}{|c|c|c|c|}
%\hline
%Site Type	&	Used	&	Available	&	Util \\\hline
%Slice LUTs 	&	43167	&	53200		&	81.14 \% \\\hline
%Block RAM Tile	&131.5 	&	140			&	93.93 \% \\\hline
%DSPs		&	64		&	220 		&	29.09 \% \\\hline
%\end{tabular}

\begin{tabular}{|c|c|c|c|}
\hline
Network Type	&	Normal	&	Quad	&	Quad-Approx \\\hline
\textbf{Resources} & & & \\\hline
Slice LUTs 	&	24771	&	22945		&	29743 \\\hline
Block RAM 	&120 	&	84		&	84 \\\hline
DSPs		&	221		&	226 		&	82\\\hline
\textbf{Performance} & & & \\\hline
\textbf{Precision} &  1x & 1x & 1x \\\hline
\textbf{Cycles for DOT}		&	9		&	9 		&	4\\\hline
\textbf{Execution time(ms)}		&	1x	&	1x	&	1.2x\\\hline
\textbf{Feature/Weight Compression} &  1x & 5.33x & 5.33x \\\hline
%\textbf{Precision $\times$ performance} & 1x & 1x & 1.2x \\\hline
\end{tabular}

